Polynomial-Time, Semantically-Secure Encryption Achieving the Secrecy Capacity

In the wiretap channel setting, one aims to get information-theoretic privacy of communicated data based only on the assumption that the channel from sender to receiver is noisier than the one from sender to adversary. The secrecy capacity is the optimal (highest possible) rate of a secure scheme, and the existence of schemes achieving it has been shown. For thirty years the ultimate and unreached goal has been to achieve this optimal rate with a scheme that is polynomial-time. (This means both encryption and decryption are proven polynomial time algorithms.) This paper finally delivers such a scheme. In fact it does more. Our scheme not only meets the classical notion of security from the wiretap literature, called MIS-R (mutual information security for random messages) but achieves the strictly stronger notion of semantic security, thus delivering more in terms of security without loss of rate.

==> preliminaries.tex <==
\section{Preliminaries}\label{sec-defs}

\heading{Basic notation and definitions.}  If $s$ is a binary string
then $s[i]$ denotes its $i$-th bit and $|s|$ denotes its length. If
$S$ is a set then $|S|$ denotes its size. If $x$ is a real number then
$|x|$ denotes its absolute value.  If $s_1, \ldots,s_l$ are strings
then $s_1\|\cdots\|s_l$ denotes their concatenation.  If $s$ is a
string and $n$ a non-negative integer then $s^n$ denotes the
concatenation of $n$ copies of $s$.  

A probability distribution is a function $P$ that associates to each
$x$ a probability $P(x)\in [0,1]$. The support $\support(P)$ is the
set of all $x$ such that $P(x)>0$. All probability distributions in
this paper are discrete. Associate to random variable $\rv{X}$ and
event $E$ the probability distributions $\pdist{X},\pdist{X|E}$
defined for all $x$ by $\pdist{\rv{X}}(x) = \Prob{\rv{X}=x}$ and
$\pdist{\rv{X}|E}(x) = \CondProb{\rv{X}=x}{E}$.  We denote by
$\lg(\cdot)$ the logarithm in base two, and by $\ln(\cdot)$ the
natural logarithm.  We adopt standard conventions such as $0\lg 0 =
0\lg\infty = 0$ and $\Pr[E_1|E_2]=0$ when $\Pr[E_2]=0$.  The function
$h\Colon [0,1]\to [0,1]$ is defined by $h(x)= - x\lg x$.  The
(Shannon) entropy of probability distribution $P$ is defined by
$\entropy(P) = \sum_x h(P(x))$ and the statistical difference between
probability distributions $P,Q$ is defined by $\SD(P;Q) = 0.5\cdot
\sum_x |P(x)-Q(x)|$.  If $\rv{X},\rv{Y}$ are random variables the
(Shannon) entropy is defined by $\entropy(\rv{X}) =
\entropy(\pdist{\rv{X}}) = \sum_x h(\pdist{\rv{X}}(x))$.  The
conditional entropy is defined via $\condentropy{\rv{X}}{\rv{Y}=y} =
\sum_x h(\pdist{\rv{X}|\rv{Y}=y}(x))$ and
$\condentropy{\rv{X}}{\rv{Y}} = \sum_y \pdist{\rv{Y}}(y)\cdot
\condentropy{\rv{X}}{\rv{Y}=y}$. The statistical or variational
distance between random variables $\rv{X_1}, \rv{X_2}$ is $
\SD(\rv{X_1};\rv{X_2}) = \SD(\pdist{\rv{X_1}};\pdist{\rv{X_2}}) =
0.5\cdot \sum_x |\Pr[\rv{X_1}=x]-\Pr[\rv{X_2}=x]|$.  The min-entropy
of random variable $\rv{X}$ is $\entropy_\infty(\rv{X})=\max_x
\Pr[\rv{X}=x]$ and if $\rv{Z}$ is also a random variable the
conditional min-entropy is $\entropy_\infty(\rv{X}|\rv{Z})=\sum_z
\Pr[\rv{Z}=z] \max_x \Pr[\rv{X}=x|\rv{Z}=z]$.

\heading{Transforms, channels and algorithms.}  We say that $T$ is a
transform with domain $D$ and range $R$, written $T\Colon D\to R$, if
$T(x)$ is a random variable over $R$ for every $x\in D$. Thus, $T$ is
fully specified by a sequence $P=\{P_x\}_{x\in D}$ of probability
distributions over $R$, where $ P_x(y) = \Pr[T(x)=y]$ for all $x\in D$
and $y\in R$. We call $P$ the distribution associated to $T$. This
distribution can be specified by a $|D|$ by $|R|$ transition
probability matrix $W$ defined by $W[x,y]=P_x(y)$.  A (randomized)
algorithm is also a transform.  Finally, an adversary too is a
transform.

\heading{Channels.} A channel is, again, just a transform.  In more
conventional communications terminology, a channel $\Ch\Colon D \to R$
has input alphabet $D$ and output alphabet $R$.

If $\ChB\Colon D\to Z$ is a channel and $c\geq 1$ is an integer we define the
channel $\ChB^c \Colon\bits^c\to Z^c$ by $\ChB^c(X)=\ChB(X[1])\Concat\cdots
\Concat\ChB(X[c])$ for all $X=X[1]\ldots X[c]\in\bits^c$. The applications of
$\ChB$ are all independent, meaning that if $W$ is the transition probability
matrix of $\ChB$ then the transition probability matrix $W_c$ of $\ChB^c$ is
defined by $W[X,Y] = W[X[1],Y[1]]\cdot \ldots \cdot W[X[c],Y[c]]$ for all
$X=X[1]\ldots X[c]\in\bits^c$ and $Y=Y[1]\ldots Y[c]\in Z^c$. We say that a
channel $\Ch$ is binary if it equals $\ChB^c$ for some channel $\ChB$ and some
$c$, in which case we refer to $\ChB$ as the base (binary) channel and $\Ch$ as
the channel induced by $\ChB$.

By $\BSC_p\Colon\bits\to\bits$ we denote the binary symmetric channel with
crossover probability $p$ ($0\leq p\leq 1/2$). Its transition probability
matrix $W$ has $W[x,y]=p$ if $x\neq y$ and $1-p$ otherwise for all
$x,y\in\bits$. The induced channel $\BSC_p^c$ flips each input bit
independently with probability $p$.

The receiver and adversary channels of the wiretap setting will have domain
$\bits^c$, where $c$ is the length of the sender ciphertext, and range
$\bits^d$, where the output length $d$ may differ between the two channels.
Such channels may be binary, which is the most natural example, but our
equivalences between security notions hold for all channels, even ones
that are not binary. 

If $\Ch1\Colon\bits^{c_1}\to\bits^{d_1}$ and
$\Ch2\Colon\bits^{c_2}\to\bits^{d_2}$ are channels then
$\Ch1\Concat\Ch2$ denotes the channel
$\Ch\Colon\bits^{c_1+c_2}\to\bits^{d_1+d_2}$ defined by
$\Ch(x_1\Concat x_2)=\Ch1(x_1)\Concat\Ch2(x_2)$ for all
$x_1\in\bits^{c_1}$ and $x_2\in\bits^{c_2}$.

Finally, we say that a channel $\Ch\Colon D \to R$ with transition
matrix $W$ is {\em symmetric} if the there exists a partition of the
range as $R = R_1 \cup \cdots \cup R_n$ such that for all $i$ the
sub-matrix $W[\cdot, R_i]$ induced by the rows in $R_i$ is strongly
symmetric, i.e., all rows are permutations of each other, and all
columns are permutations of each other.



